Fast and Compact Sketch-Based Dynamic Connectivity

We study the dynamic connectivity problem for massive, dense graphs. Our goal is to build a system for dense graphs that simultaneously answers connectivity queries quickly, maintains a fast update throughput, and a uses a small amount of memory. Existing systems at best achieve two of these three performance goals at once. We present a parallel dynamic connectivity algorithm using graph sketching techniques that has space complexity $O(V \log^3 V)$ and query complexity $O(\log V/\log\log V)$. Its updates are fast and parallel: in the worst case, it performs updates in $O(\log^2 V)$ depth and $O(\log^4 V)$ work. For updates which don't change the spanning forests maintained by our data structure, the update complexity is $O(\log V)$ depth and $O(\log^2 V)$ work. We also present CUPCaKE (Compact Updating Parallel Connectivity and Sketching Engine), a dynamic connectivity system based on our parallel algorithm. It uses an order of magnitude less memory than the best lossless systems on dense graph inputs, answers queries with microsecond latency, and ingests millions of updates per second on dense graphs.

==> 07_related.tex <==
\section{Related Work}\label{sec:related}

\begin{comment}
    
\myparagraph{Dynamic Connectivity Algorithms}
Henzinger and King~\cite{conn_apps} achieve the first algorithm with polylogarithmic update time: $O(\log^3 \nodesize)$ amortized update time and $O(\log\nodesize/\log\log\nodesize)$ worst-case query time. Subsequent work~\cite{henzinger1997sampling,holm2001poly} has improved the update cost multiple times, and the best known algorithm with $O(\log\nodesize/\log\log\nodesize)$ queries has $O(\log^2 \nodesize/ (\log\log\nodesize))$ amortized update time~\cite{wulff2013faster}. There are also several algorithms with query time $O(\log\nodesize/\log\log\log\nodesize)$~\cite{thorup2000near}; the best has amortized update time $O(\log\nodesize(\log\log\nodesize)^2)$~\cite{huang2023fully}.
\end{comment}

\myparagraph{Dynamic Connectivity Implementations}
In this paper we have reviewed \cdcname~\cite{chen2022dynamic} and \dtree~\cite{fedorov2021scalable}, two systems for solving dynamic connectivity which are based on lossless algorithms. In the closely related batch-dynamic model, edge updates arrive in batches of exclusively insertions or deletions, and batch size parametrizes system performance. Notable batch-dynamic systems that solve connectivity include Aspen~\cite{aspen} and Terrace~\cite{terrace}.


\myparagraph{Graph Sketching Algorithms}
Ahn \etal~\cite{Ahn2012} introduced seminal connectivity sketch algorithm, which subsequent work~\cite{nelson2019optimal} has shown to be space-optimal. Since then, results for many graph problems have been found, including matchings~\cite{ChitnisCEHMMV16}, triangle counting~\cite{McGregorVV16}, cut and spectral sparsification~\cite{AhnGM13,KapralovLMMS13,KapralovW14}, vertex connectivity~\cite{GuhaMT15}, densest subgraph,~\cite{McGregorTVV15} and correlation clustering~\cite{clustering}.

\myparagraph{Graph Sketching Systems}
In this paper we have reviewed some components of GraphZeppelin~\cite{tench2024graphzeppelin} and Landscape~\cite{landscape}, the only existing implementations of connectivity sketching algorithms. GraphZeppelin is a single-machine system that uses solid state drives to increase the scale of graphs it can process. Landscape is a distributed implementation which stores the graph sketch on a main node and distributes the computational work of computing sketch updates to a cluster of stateless worker nodes.

==> acknowledgements.tex <==

\myparagraph{Acknowledgements}
\evan{Add seawulf and associated grants to acknowledgement}
The authors would like to thank Stony Brook Research Computing and Cyberinfrastructure and the Institute for Advanced Computational Science at Stony Brook University for access to the high-performance SeaWulf computing system, which was made possible by \$1.85M in grants from the National Science Foundation (awards 1531492 and 2215987) and matching funds from the Empire State Development’s Division of Science, Technology and Innovation (NYSTAR) program (contract C210148).

==> copyright.tex <==
\copyrightyear{2021}
\acmYear{2022}
\setcopyright{acmlicensed}
\acmConference[SIGMOD '22]{SIGMOD '22: ACM  Special Interest Group on Management of Data}{June 12--17, 2022}{Philadelphia, PA}
\acmBooktitle{SIGMOD '22: ACM  Special Interest Group on Management of Data, June 12--17, 2022, Philadelphia, PA}
\acmPrice{15.00}
\acmDOI{10.1145/3448016.3457313}
\acmISBN{78-1-4503-8343-1/21/06}

==> figures/cameo-figure.tex <==
\begin{figure}[ht]
    \centering
\includegraphics[width=0.7\linewidth]{sigmod_paper/figures/images/cameosketch-diagram.png}
    \caption{An illustration of a single Cameo Sketch. The sketch consists of $O(1)$ columns each containing $O(\log^2 V)$ bits where $V^2$ is the length of the vector being sketched. Cameo Sketch supports updates in $O(1)$ time. See Theorem \ref{thm:cameosketch}.}
    \label{fig:cameo}
\end{figure}

\daniel{Talk about this figure in the text. Or delete it. Maybe we don't describe Cameo Sketch}

==> figures/ett-figure.tex <==
\begin{figure}[ht]
    \centering
\includegraphics[width=\linewidth]{sigmod_paper/figures/images/ETT-diagram-2.png}
    \caption{This figure illustrates the $O(\log \nodesize)$ levels of our data structure. Each level consists of a reduced height Euler tour tree. Each node in the skip list marked with a square is augmented with a single Cameo Sketch (see Figure~\ref{fig:cameo}). Note that some of the bottom level nodes do not contain sketches due to a space optimization described later in Section~\ref{sec:perf_eng}.}
    \label{fig:ett}
\end{figure}

\daniel{Fix the text size}
\daniel{Consider a two-column figure}
\daniel{Talk about this figure in the text}
\daniel{Talk about representative vertex}

==> figures/linkcut-figure.tex <==
\begin{figure}[ht]
    \centering
\includegraphics[width=\linewidth]{sigmod_paper/figures/images/linkcut-diagram.png}
    \caption{This figure shows the link-cut tree and reduced height Euler tour tree. These data structures exist on the input node to find cycle edges (link-cut tree) and answer connectivity queries (Euler tour tree) respectively.}
    \label{fig:linkcut}
\end{figure}


\daniel{Talk about this figure in the text}

==> lemmas/rh_alg.tex <==
\begin{theorem}\label{thm:rh_alg}
    For a graph $\graph=(\nodes,\edges)$, there exists a dynamic connectivity algorithm that performs normal updates in worst-case $O(\log^2 \nodesize / \log\log \nodesize)$ time and performs isolated updates in worst-case $O(\log^5 \nodesize)$ time.
\end{theorem}

==> lemmas/rh_cutset.tex <==
\begin{lemma}\label{lem:rh_cutset}
    For a graph $\graph = (\nodes, \edges)$ and a forest $\forest = (\nodes, \edges_{\forest} \subseteq \edges)$ there exists a cutset data structure that performs $\update$ operations in $O(\log \nodesize / \log\log \nodesize)$ time and performs $\link$ and $\cut$ operations in $O(\log^3 \nodesize)$ time, and performs $\query$ operations in $O(\log \nodesize / \log\log \nodesize)$ time.
\end{lemma}

==> lemmas/rh_par_alg.tex <==
\begin{theorem}\label{thm:rh_par_alg}
    For a graph $\graph=(\nodes,\edges)$ there exists a dynamic connectivity algorithm that performs normal updates in $O(\log \nodesize / \log\log \nodesize)$ depth and $O(\log^2 \nodesize / \log\log \nodesize)$ work and performs isolated updates in $O(\log^3 \nodesize)$ depth and $O(\log^5 \nodesize)$ work in the binary fork-join model.
\end{theorem}

==> lemmas/rh_par_cutset.tex <==
\begin{lemma}\label{lem:rh_par_cutset}
    For a graph $\graph = (\nodes, \edges)$ and a forest $\forest = (\nodes, \edges_{\forest} \subseteq \edges)$ there exists a cutset data structure that performs $\link$ and $\cut$ operations in $O(\log^2 \nodesize)$ depth and $O(\log^3 \nodesize)$ work in the binary fork-join model, performs $\update$ operations in $O(\log \nodesize / \log\log \nodesize)$ time, and performs $\query$ operations in $O(\log \nodesize / \log\log \nodesize)$ time.
\end{lemma}

